The debt aversion survey module: An experimentally validated tool to measure individual debt aversion

We develop an experimentally validated, short and easy-to-use survey module for measuring individual debt aversion. To this end, we first estimate debt aversion on an individual level, using choice data from Meissner and Albrecht (2022). This data also contains responses to a large set of debt aversion survey items, consisting of existing items from the literature and novel items developed for this study. Out of these, we identify a survey module comprising two qualitative survey items to best predict debt aversion in the incentivized experiment.

==> DSM_(arxiv)/FIGURES/fig.example_questionnaire.tex <==

\begin{figure}[h]
    \begin{center}
        \fboxsep=12pt
        \fbox{
        \begin{minipage}{0.8\textwidth}
        Please rate the following statement.\bigbreak
        
        \hspace{12pt}\textit{\textbf{Debt is an integral part of today's life.}}\vspace{-12pt}
        
            \begin{center}
            \begin{tabular}{c c c c c c}
                 {\small strongly agree \hspace{6pt} $\square$}
                 & {\small $\square$}
                 & {\small $\square$}
                 & {\small $\square$}
                 & {\small $\boxtimes$}
                 & {\small $\square$ \hspace{6pt} strongly disagree }
            \end{tabular}
            \end{center}
        
%        \hspace{12pt}\textit{\textbf{I feel OK borrowing money for `essential' purchases e.g. cars, appliances, mortgage.}}\vspace{-12pt}
            
%            \begin{center}
%            \begin{tabular}{c c c c c c}
%                 {\small very much like me \hspace{6pt} $\square$}
%                 & {\small $\square$}
%                 & {\small $\square$}
%                 & {\small $\boxtimes$}
%                 & {\small $\square$}
%                 & {\small $\square$ \hspace{6pt} not at all like me }\\
%            \end{tabular}
%            \end{center}
            
        \begin{center} --- \end{center}
        
        What do you think how does the average participant in this survey/experiment rate the following statement?\bigbreak
        
        \hspace{12pt}\textit{\textbf{There is no excuse for borrowing money.}}\vspace{-12pt}
        
            \begin{center}
            \begin{tabular}{c c c c c c}
                 {\small strongly agree \hspace{6pt} $\square$}
                 & {\small $\boxtimes$}
                 & {\small $\square$}
                 & {\small $\square$}
                 & {\small $\square$}
                 & {\small $\square$ \hspace{6pt} strongly disagree }\\
            \end{tabular}
            \end{center}
        
        \end{minipage}
        }
    \end{center}

\caption{Debt aversion survey module answered by a hypothetical respondent}
\label{fig.example_questionnaire}
\end{figure}

==> DSM_(arxiv)/FIGURES/fig.gamma_hist.tex <==

\begin{figure}
\caption{Individual level estimates of the debt aversion parameter $\gamma$. \label{figure.indiv_parameter_freq}}
\centering
\begin{tikzpicture}
\begin{axis}[
	width  = 0.8*\textwidth,
	height = 5cm,
	ybar,
	ymin=0,
	ymax=28,
	axis lines = left,
	ylabel = no. of individuals,
	ymajorgrids = true,
	xmin = 0.9,
	xmax = 1.175,
	xlabel= debt aversion ($\gamma$),
	xtick = data,
	extra x ticks={1},
	extra x tick style={xticklabel=1},
	xticklabels={,,0.95,,1,,1.05,,1.1,,1.15,},
	area style,
]

\addplot+[ybar interval,mark=no,] plot coordinates {	
                                                    (0.9, 0) 
													(0.925, 1)
													(0.95, 1)
													(0.975, 2)
													(1.0, 16)
													(1.025, 24)
													(1.05, 24)
												    (1.075, 20)
													(1.1, 8)
													(1.125, 0)
													(1.15, 0)
													%(1.175, 0)
													};

\end{axis}
\end{tikzpicture}

%\flushleft
%\footnotesize
%\floatfoot{Notes: Estimates are retrieved through hierarchical maximum likelihood procedures based on observed choices and the population distribution of preference parameters. The relative influence of population distribution as opposed to individual choices during estimation is controlled through the shrinkage factor $s=0.00076$, which has been set in order to optimize estimation accuracy of $\gamma$ based on simulations.}
\end{figure}

==> DSM_(arxiv)/FIGURES/fig.module_selection.tex <==
\begin{figure}[t!]
\caption{Performance metrics of the candidate survey modules
\label{fig.performance}}


\begin{subfigure}{1\textwidth}
\begin{minipage}{0.49\textwidth}
\begin{tikzpicture}
\centering
    \hspace{9pt}
	%%%%% COEFFICIENT OF DETERMINATION
	\begin{axis}[
		width  = 0.95*\textwidth,
		height = 5.5cm,
		ymin=0,
		ymax=0.25,
		axis lines = left,
		ylabel = \footnotesize{$R^2$},
		ymajorgrids = true,
		xmin = 0,
		xmax = 13,
		tick label style={font=\footnotesize},
		legend entries={\scriptsize{Top1}, \scriptsize{Top2}, \scriptsize{Top3},
        \scriptsize{Top4}, \scriptsize{Top5}},
        legend style={at={(0.975,0.65)}},
		%xlabel= No. of predictors,
		]
        \addplot [red,very thick] table [x="n_tuple", 
                                        y="r.squared.1", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [darkgray] table [x="n_tuple", 
                               y="r.squared.2",
                               col sep=comma, 
                               mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray] table [x="n_tuple", 
                               y="r.squared.3",
                               col sep=comma, 
                               mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray, densely dotted] table [x="n_tuple",
                               y="r.squared.4", 
                               col sep=comma, 
                               mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [lightgray, dotted] table [x="n_tuple",
                               y="r.squared.5",
                               col sep=comma, 
                               mark=none] {RESULTS/survey_module_selection.csv};
	\end{axis}
\end{tikzpicture}
\end{minipage}
%
\begin{minipage}{0.49\textwidth}
\begin{tikzpicture}
\centering
    \hspace{9pt}
	%%%%% ADJUSTED COEFFICIENT OF DETERMINATION
	\begin{axis}[
		width  = 0.95*\textwidth,
		height = 5.5cm,
		ymin=0,
		ymax=0.25,
		axis lines = left,
		ylabel = \footnotesize{adjusted $R^2$},
		ymajorgrids = true,
		xmin = 0,
		xmax = 13,
		tick label style={font=\footnotesize},
		%xlabel= No. of predictors,
		]
        \addplot [red,very thick] table [x="n_tuple", 
                                        y="adj.r.squared.1", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [darkgray] table [x="n_tuple",
                                        y="adj.r.squared.2", 
                                        col sep=comma, 
                               mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray] table [x="n_tuple", 
                                        y="adj.r.squared.3", 
                                        col sep=comma, 
                               mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray, densely dotted] table [x="n_tuple",
                                        y="adj.r.squared.4", 
                                        col sep=comma, 
                               mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [lightgray, dotted] table [x="n_tuple",
                                        y="adj.r.squared.5", 
                                        col sep=comma, 
                               mark=none] {RESULTS/survey_module_selection.csv};
       \addplot[blue, ultra thick, draw opacity=0.1]coordinates{(9,0) (9,0.142844833311355)};
	\end{axis}
\end{tikzpicture}
\end{minipage}
\end{subfigure}

\vspace{1cm}
\begin{subfigure}{1\textwidth}
\begin{minipage}{0.49\textwidth}
\begin{tikzpicture}
\centering
	%%%%% AKAIKE INFORMATION CRITERION
	\begin{axis}[
		width  = 0.95*\textwidth,
		height = 5.5cm,
		ymin=-658,
		ymax=-647,
		axis lines = left,
		ylabel = \footnotesize{AIC},
		ymajorgrids = true,
		xmin = 0,
		xmax = 13,
		tick label style={font=\footnotesize}
		%xlabel= No. of predictors,
		]
        \addplot [red,very thick] table [x="n_tuple",
                                        y="AIC.1", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [darkgray] table [x="n_tuple",
                                        y="AIC.2", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray] table [x="n_tuple",
                                        y="AIC.3", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray, densely dotted] table [x="n_tuple", 
                                        y="AIC.4", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [lightgray, dotted] table [x="n_tuple", 
                                        y="AIC.5", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot[blue, ultra thick, draw opacity=0.1]coordinates{(6,-661) (6,-656.477233123315)};
	\end{axis}
\end{tikzpicture}
\end{minipage}
%
\begin{minipage}{0.49\textwidth}
\begin{tikzpicture}
\centering
	%%%%% BAYESIAN INFORMATION CRITERION
	\begin{axis}[
		width  = 0.95*\textwidth,
		height = 5.5cm,
		ymin=-652,
		ymax=-608,
		axis lines = left,
		ylabel = \footnotesize{BIC},
		ymajorgrids = true,
		xmin = 0,
		xmax = 13,
		tick label style={font=\footnotesize}
		%xlabel= No. of predictors,
		]
        \addplot [red,very thick] table [x="n_tuple", 
                                        y="BIC.1", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [darkgray] table [x="n_tuple", 
                                        y="BIC.2", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray] table [x="n_tuple", 
                                        y="BIC.3", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray, densely dotted] table [x="n_tuple", 
                                        y="BIC.4", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [lightgray, dotted] table [x="n_tuple", 
                                        y="BIC.5", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot[blue, ultra thick, draw opacity=0.1]coordinates{(1,-652) (1,-647.056288196309)};
	\end{axis}
\end{tikzpicture}
\end{minipage}
\end{subfigure}
\vspace{1cm}
\begin{comment}
\begin{subfigure}{1\textwidth}
\begin{minipage}{0.49\textwidth}
\begin{tikzpicture}
\centering
	%%%%% CROSS VALIDATION (k=5)
	\begin{axis}[
		width  = 0.95*\textwidth,
		height = 5cm,
		ymin=0.001,
		ymax=0.031,
		axis lines = left,
		ylabel = \footnotesize{MAE (CV with k=5)},
		ymajorgrids = true,
		xmin = 0,
		xmax = 16,
		xlabel= No. of predictors,
		scaled ticks=false, 
		tick label style={font=\footnotesize},
		y tick label style={/pgf/number format/.cd,
        fixed,
        fixed zerofill,
        precision=4,
        %yticklabels={,,.030,.031,.032},
        %/tikz/.cd
        }
		]
        \addplot [red,very thick] table [x="n_tuple", 
                                        y="MAE_k5_rd100.1", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [darkgray] table [x="n_tuple", 
                                        y="MAE_k5_rd100.2", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray] table [x="n_tuple", 
                                        y="MAE_k5_rd100.3", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray, densely dotted] table [x="n_tuple", 
                                        y="MAE_k5_rd100.4", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [lightgray, dotted] table [x="n_tuple", 
                                        y="MAE_k5_rd100.5", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
	\end{axis}
\end{tikzpicture}
\end{minipage}
%
\begin{minipage}{0.49\textwidth}
\begin{tikzpicture}
\centering
	%%%%% CROSS VALIDATION (k=10)
	\begin{axis}[
		width  = 0.95*\textwidth,
		height = 5cm,
		ymin=0.02,
		ymax=0.031,
		axis lines = left,
		ylabel = \footnotesize{MAE (CV with k=10)},
		ymajorgrids = true,
		xmin = 0,
		xmax = 16,
		xlabel= No. of predictors,
		scaled ticks=false, 
		tick label style={font=\footnotesize},
		y tick label style={/pgf/number format/.cd,
        fixed,
        fixed zerofill,
        precision=4,
        %yticklabels={,,.030,.031,.032},
        %/tikz/.cd
        }
		]
        \addplot [red,very thick] table [x="n_tuple", 
                                        y="MAE_k10_rd100.1", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [darkgray] table [x="n_tuple", 
                                        y="MAE_k10_rd100.2", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray] table [x="n_tuple", 
                                        y="MAE_k10_rd100.3", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray, densely dotted] table [x="n_tuple", 
                                        y="MAE_k10_rd100.4", 
                                        col sep=comma,
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [lightgray, dotted] table [x="n_tuple", 
                                        y="MAE_k10_rd100.5", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
	\end{axis}
\end{tikzpicture}
\end{minipage}
\end{subfigure}
\end{comment}

\begin{subfigure}{1\textwidth}
\begin{minipage}{0.49\textwidth}
\begin{tikzpicture}
\centering
	%%%%% CROSS VALIDATION (k=5)
	\begin{axis}[
		width  = 0.95*\textwidth,
		height = 5.5cm,
		ymin=0.00105,
		ymax=0.00135,
		axis lines = left,
		ylabel = \footnotesize{MSE (CV with k=5)},
		ymajorgrids = true,
		xmin = 0,
		xmax = 13,
		xlabel= No. of predictors,
		scaled ticks=false, 
		tick label style={font=\footnotesize},
		y tick label style={/pgf/number format/.cd,
        fixed,
        fixed zerofill,
        precision=4,
        yticklabels={,,.0011,.0012,.0013,,},
        /tikz/.cd
        }
		]
        \addplot [red,very thick] table [x="n_tuple", 
                                        y="MSPE_k5_rd100.1", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [darkgray] table [x="n_tuple", 
                                        y="MSPE_k5_rd100.2", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray] table [x="n_tuple", 
                                        y="MSPE_k5_rd100.3", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray, densely dotted] table [x="n_tuple", 
                                        y="MSPE_k5_rd100.4", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [lightgray, dotted] table [x="n_tuple", 
                                        y="MSPE_k5_rd100.5", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot[blue, ultra thick, draw opacity=0.1]coordinates{(2,0.00110130341633874) (2,0.00105)};
	\end{axis}
\end{tikzpicture}
\end{minipage}
%
\begin{minipage}{0.49\textwidth}
\begin{tikzpicture}
\centering
	%%%%% CROSS VALIDATION (k=10)
	\begin{axis}[
		width  = 0.95*\textwidth,
		height = 5.5cm,
		ymin=0.00105,
		ymax=0.00135,
		axis lines = left,
		ylabel = \footnotesize{MSE (CV with k=10)},
		ymajorgrids = true,
		xmin = 0,
		xmax = 13,
		xlabel= No. of predictors,
		scaled ticks=false, 
		tick label style={font=\footnotesize},
		y tick label style={/pgf/number format/.cd,
        fixed,
        fixed zerofill,
        precision=4,
        yticklabels={,,.0011,.0012,.0013,,},
        /tikz/.cd
        }
		]
        \addplot [red,very thick] table [x="n_tuple", 
                                        y="MSPE_k10_rd100.1", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [darkgray] table [x="n_tuple", 
                                        y="MSPE_k10_rd100.2", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray] table [x="n_tuple", 
                                        y="MSPE_k10_rd100.3", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray, densely dotted] table [x="n_tuple", 
                                        y="MSPE_k10_rd100.4", 
                                        col sep=comma,
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [lightgray, dotted] table [x="n_tuple", 
                                        y="MSPE_k10_rd100.5", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot[blue, ultra thick, draw opacity=0.1]coordinates{(2,0.00109987097281651) (2,0.00105)};
	\end{axis}
\end{tikzpicture}
\end{minipage}
\end{subfigure}

\vspace{0.5cm}
\footnotesize

\footnotesize{Notes: \textbf{First row:} coefficients of determination;
\textbf{Second row:} information criteria;
\textbf{Third row:} mean squared error (MSE) derived through k-fold cross validation (CV) with $k=5$ and $k=10$ data chunks and 100 repetitions each}
\end{figure}

==> DSM_(arxiv)/FIGURES/fig.module_selection_slides.tex <==
\begin{figure}[t!]
%\caption{Performance metrics of the candidate survey modules
%\label{fig.performance}}


\begin{subfigure}{1\textwidth}
\begin{minipage}{0.49\textwidth}
\begin{tikzpicture}
\centering
    \hspace{9pt}
	%%%%% ADJUSTED COEFFICIENT OF DETERMINATION
	\begin{axis}[
		width  = 0.95*\textwidth,
		height = 5.5cm,
		ymin=0,
		ymax=0.5,
		axis lines = left,
		ylabel = \footnotesize{adjusted $R^2$},
		ymajorgrids = true,
		xmin = 0,
		xmax = 16,
		tick label style={font=\footnotesize},
		%xlabel= No. of predictors,
		]
        \addplot [red,very thick] table [x="n_tuple", 
                                        y="adj.r.squared.1", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [darkgray] table [x="n_tuple",
                                        y="adj.r.squared.2", 
                                        col sep=comma, 
                               mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray] table [x="n_tuple", 
                                        y="adj.r.squared.3", 
                                        col sep=comma, 
                               mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray, densely dotted] table [x="n_tuple",
                                        y="adj.r.squared.4", 
                                        col sep=comma, 
                               mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [lightgray, dotted] table [x="n_tuple",
                                        y="adj.r.squared.5", 
                                        col sep=comma, 
                               mark=none] {RESULTS/survey_module_selection.csv};
        \addplot[blue, ultra thick, draw opacity=0.1]coordinates{(13,0) (13,0.361038)};
	\end{axis}
\end{tikzpicture}
\end{minipage}
%
\begin{minipage}{0.49\textwidth}
\begin{tikzpicture}
\centering
    \hspace{9pt}
	%%%%% AKAIKE INFORMATION CRITERION
	\begin{axis}[
		width  = 0.95*\textwidth,
		height = 5.5cm,
		ymin=-570,
		ymax=-542,
		axis lines = left,
		ylabel = \footnotesize{AIC},
		ymajorgrids = true,
		xmin = 0,
		xmax = 16,
		tick label style={font=\footnotesize},
		legend entries={\scriptsize{Top1}, \scriptsize{Top2},                                    \scriptsize{Top3},
                        \scriptsize{Top4}, \scriptsize{Top5}},
        legend style={at={(0.975,0.975)}},
		%xlabel= No. of predictors,
		]
        \addplot [red,very thick] table [x="n_tuple",
                                        y="AIC.1", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [darkgray] table [x="n_tuple",
                                        y="AIC.2", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray] table [x="n_tuple",
                                        y="AIC.3", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray, densely dotted] table [x="n_tuple", 
                                        y="AIC.4", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [lightgray, dotted] table [x="n_tuple", 
                                        y="AIC.5", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot[blue, ultra thick, draw opacity=0.1]coordinates{(10,-570) (10,-565.841)};
	\end{axis}
\end{tikzpicture}
\end{minipage}
\end{subfigure}

\vspace{1cm}
\begin{subfigure}{1\textwidth}
\begin{minipage}{0.49\textwidth}
\begin{tikzpicture}
\centering
	%%%%% BAYESIAN INFORMATION CRITERION
	\begin{axis}[
		width  = 0.95*\textwidth,
		height = 5.5cm,
		ymin=-548,
		ymax=-523,
		xlabel= No. of predictors,
		axis lines = left,
		ylabel = \footnotesize{BIC},
		ymajorgrids = true,
		xmin = 0,
		xmax = 16,
		tick label style={font=\footnotesize}
		%xlabel= No. of predictors,
		]
        \addplot [red,very thick] table [x="n_tuple", 
                                        y="BIC.1", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [darkgray] table [x="n_tuple", 
                                        y="BIC.2", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray] table [x="n_tuple", 
                                        y="BIC.3", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray, densely dotted] table [x="n_tuple", 
                                        y="BIC.4", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [lightgray, dotted] table [x="n_tuple", 
                                        y="BIC.5", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot[blue, ultra thick, draw opacity=0.1]coordinates{(1,-548) (1,-544.05)};
	\end{axis}
\end{tikzpicture}
\end{minipage}
%
\begin{minipage}{0.49\textwidth}
\begin{tikzpicture}
\centering
	%%%%% CROSS VALIDATION (k=10)
	\begin{axis}[
		width  = 0.95*\textwidth,
		height = 5.5cm,
		ymin=0.0006,
		ymax=0.00089,
		axis lines = left,
		ylabel = \footnotesize{MSE (CV with k=10)},
		ymajorgrids = true,
		xmin = 0,
		xmax = 16,
		xlabel= No. of predictors,
		scaled ticks=false, 
		tick label style={font=\footnotesize},
		y tick label style={/pgf/number format/.cd,
        fixed,
        fixed zerofill,
        precision=4,
        yticklabels={,,.0007,.0008,},
        /tikz/.cd
        }
		]
        \addplot [red,very thick] table [x="n_tuple", 
                                        y="MSPE_k10_rd100.1", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [darkgray] table [x="n_tuple", 
                                        y="MSPE_k10_rd100.2", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray] table [x="n_tuple", 
                                        y="MSPE_k10_rd100.3", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray, densely dotted] table [x="n_tuple", 
                                        y="MSPE_k10_rd100.4", 
                                        col sep=comma,
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [lightgray, dotted] table [x="n_tuple", 
                                        y="MSPE_k10_rd100.5", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot[blue, ultra thick, draw opacity=0.1]coordinates{(8,0.000664) (8,0.0006)};
	\end{axis}
\end{tikzpicture}
\end{minipage}
\end{subfigure}
\vspace{1cm}
\end{figure}

==> DSM_(arxiv)/TABLES/tab.MPLs.tex <==
\begin{table}[htp]
\begin{tabularx}{\textwidth}{ 
    c
    @{\hspace{36pt}}
  >{\centering\arraybackslash}X 
  >{\centering\arraybackslash}X 
  }
\toprule

\textbf{Choice} 
& \textbf{Option A}
& \textbf{Option B}\\
\hline

\footnotesize{1}
& \footnotesize{Receive an amount of \euro{18.2} today}
& \footnotesize{Receive an amount of  \euro{18.0} in 4 weeks}\\

\footnotesize{2}
& \footnotesize{Receive an amount of \euro{18.0} today}
& \footnotesize{Receive an amount of  \euro{18.0} in 4 weeks}\\

\footnotesize{3} 
& \footnotesize{Receive an amount of  \euro{17.8} today} 
& \footnotesize{Receive an amount of  \euro{18.0} in 4 weeks}\\

\footnotesize{4}
& \footnotesize{Receive an amount of  \euro{17.3} today}
& \footnotesize{Receive an amount of  \euro{18.0} in 4 weeks}\\

\footnotesize{5}
& \footnotesize{Receive an amount of  \euro{16.8} today}
& \footnotesize{Receive an amount of  \euro{18.0} in 4 weeks}\\

\footnotesize{6}
& \footnotesize{Receive an amount of  \euro{16.0} today}
& \footnotesize{Receive an amount of  \euro{18.0} in 4 weeks}\\

\footnotesize{7}
& \footnotesize{Receive an amount of  \euro{14.0} today}
& \footnotesize{Receive an amount of  \euro{18.0} in 4 weeks}\\

\footnotesize{8}
& \footnotesize{Receive an amount of  \euro{12.0} today}
& \footnotesize{Receive an amount of  \euro{18.0} in 4 weeks}\\

\footnotesize{9}
& \footnotesize{Receive an amount of  \euro{10.0} today}
& \footnotesize{Receive an amount of  \euro{18.0} in 4 weeks}\\

\footnotesize{10}
& \footnotesize{Receive an amount of  \euro{8.0} today}
& \footnotesize{Receive an amount of  \euro{18.0} in 4 weeks}\\

\bottomrule
\end{tabularx}
\caption{Multiple price list of intertemporal choices (MPL1)}
\label{tab:MPLI}
\end{table}



\begin{table}[htp]
\begin{tabularx}{\textwidth}{ 
c
@{\hspace{36pt}}
C{0.1cm} 
>{\centering\arraybackslash}X 
>{\centering\arraybackslash}X 
C{0.1cm} 
>{\centering\arraybackslash}X 
>{\centering\arraybackslash}X  
C{0.1cm}
}
\toprule
& & \multicolumn{2}{c}{\textbf{Option A}} & & \multicolumn{2}{c}{\textbf{Option B}} & \\
\cline{3-4} \cline{6-7}
\textbf{Choice}  & &  \makecell{\small{ Coin shows  } \\[-0.2cm] \small{ Heads }} & \makecell*{\small{ Coin shows  } \\[-0.2cm] \small{ Tails }} & & \makecell*{\small{ Coin shows  } \\[-0.2cm] \small{ Heads }} & \makecell*{\small{ Coin shows  } \\[-0.2cm] \small{ Tails }} & \\
\hline
\footnotesize{1} & & \footnotesize{\euro{30}  today} & \footnotesize{\euro{30}  today} & & \footnotesize{\euro{30}  today} & \footnotesize{\euro{1}  today} & \\
\footnotesize{2} & & \footnotesize{\euro{25}  today} & \footnotesize{\euro{25}  today} & & \footnotesize{\euro{30}  today} & \footnotesize{\euro{1}  today} & \\
\footnotesize{3} & & \footnotesize{\euro{20}  today} & \footnotesize{\euro{20}  today} & & \footnotesize{\euro{30} today} & \footnotesize{\euro{1}  today} & \\
\footnotesize{4} & & \footnotesize{\euro{17}  today} & \footnotesize{\euro{17}  today} & & \footnotesize{\euro{30}  today} & \footnotesize{\euro{1}  today} & \\
\footnotesize{5} & & \footnotesize{\euro{16}  today} & \footnotesize{\euro{16}  today} & & \footnotesize{\euro{30}  today} & \footnotesize{\euro{1}  today} & \\
\footnotesize{6} & & \footnotesize{\euro{15}  today} & \footnotesize{\euro{15}  today} & & \footnotesize{\euro{30}  today} & \footnotesize{\euro{1} today} & \\
\footnotesize{7} & &\footnotesize{\euro{12}  today} & \footnotesize{\euro{12}  today} & & \footnotesize{\euro{30}  today} & \footnotesize{\euro{1}  today} & \\
\footnotesize{8} & & \footnotesize{\euro{10}\  today} & \footnotesize{\euro{10}  today} & & \footnotesize{\euro{30}  today} & \footnotesize{\euro{1}  today} & \\
\footnotesize{9} & &\footnotesize{\euro{5}  today} & \footnotesize{\euro{5}  today} & & \footnotesize{\euro{30}  today} & \footnotesize{\euro{1}  today} & \\
\footnotesize{10} & & \footnotesize{\euro{1}  today} & \footnotesize{\euro{1}  today} & & \footnotesize{\euro{30}  today} & \footnotesize{\euro{1}  today} &\\
\bottomrule
\end{tabularx}
\caption{Multiple price list of certain payments vs. risky gambles (MPL2)}
\label{tab:MPLII}
\end{table}


\begin{table}[htp]
\begin{tabularx}{\textwidth}{ 
c
@{\hspace{36pt}}
C{0.1cm} 
>{\centering\arraybackslash}X 
>{\centering\arraybackslash}X 
C{0.1cm} 
>{\centering\arraybackslash}X 
>{\centering\arraybackslash}X  
C{0.1cm}
}
\toprule
& & \multicolumn{2}{c}{\textbf{Option A}} & & \multicolumn{2}{c}{\textbf{Option B}} & \\
\cline{3-4} \cline{6-7}
\textbf{Choice}  & &  \makecell{\small{ Coin shows  } \\[-0.2cm] \small{ Heads }} & \makecell*{\small{ Coin shows  } \\[-0.2cm] \small{ Tails }} & & \makecell*{\small{ Coin shows  } \\[-0.2cm] \small{ Heads }} & \makecell*{\small{ Coin shows  } \\[-0.2cm] \small{ Tails }} & \\
\hline
\footnotesize{1} & & \footnotesize{\euro{14}  today} & \footnotesize{\euro{17}  today} & & \footnotesize{\euro{17}  today} & \footnotesize{\euro{1} today} & \\
\footnotesize{2} & & \footnotesize{\euro{14}  today} & \footnotesize{\euro{17}  today} & & \footnotesize{\euro{20}  today} & \footnotesize{\euro{1} today} & \\
\footnotesize{3} & & \footnotesize{\euro{14}  today} & \footnotesize{\euro{17}  today} & & \footnotesize{\euro{25}  today} & \footnotesize{\euro{1} today} & \\
\footnotesize{4} & & \footnotesize{\euro{14}  today} & \footnotesize{\euro{17} today} & & \footnotesize{\euro{28}  today} & \footnotesize{\euro{1} today} & \\
\footnotesize{5} & & \footnotesize{\euro{14}  today} & \footnotesize{\euro{17}  today} & & \footnotesize{\euro{29}  today} & \footnotesize{\euro{1} today} & \\
\footnotesize{6} & & \footnotesize{\euro{14}  today} & \footnotesize{\euro{17}  today} & & \footnotesize{\euro{30}  today} & \footnotesize{\euro{2}  today} & \\
\footnotesize{7} & &\footnotesize{\euro{14} today} & \footnotesize{\euro{17}  today} & & \footnotesize{\euro{30}  today} & \footnotesize{\euro{3}  today} & \\
\footnotesize{8} & & \footnotesize{\euro{14}  today} & \footnotesize{\euro{17}  today} & & \footnotesize{\euro{32}  today} & \footnotesize{\euro{8}  today} & \\
\footnotesize{9} & &\footnotesize{\euro{14}  today} & \footnotesize{\euro{17}  today} & & \footnotesize{\euro{32}  today} & \footnotesize{\euro{10}  today} & \\
\footnotesize{10} & & \footnotesize{\euro{14}  today} & \footnotesize{\euro{17}  today} & & \footnotesize{\euro{32}  today} & \footnotesize{\euro{14}  today} & \\
\bottomrule
\end{tabularx}
\caption{Multiple price list of less risky vs. more risky gambles (MPL3)}
\label{tab:MPLIII}
\end{table}



\begin{table}[htp]
\begin{tabularx}{\textwidth}{
    c
    @{\hspace{36pt}}
    C{0.1cm} 
  >{\centering\arraybackslash}X 
    C{0.1cm} 
  >{\centering\arraybackslash}X 
    C{0.1cm}
    }
\toprule
 & & \multicolumn{3}{c}{\textbf{Early saving contracts}} & \\
\cline{3-5}
\textbf{Choice} & & \makecell{\small{ Session 1 } \\[-0.2cm] \footnotesize{ (today) }} & & \makecell{\small{ Session 2 } \\[-0.2cm] \footnotesize{ (in 4 weeks) }} & \\

\hline
\footnotesize{1} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{45}}\\
\footnotesize{2} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{40}}\\
\footnotesize{3} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{36}}\\
\footnotesize{4} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{34}}\\
\footnotesize{5} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{32}}\\
\footnotesize{6} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{30}}\\
\footnotesize{7} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{28}}\\
\footnotesize{8} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{26}}\\
\footnotesize{9} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{24}}\\
\footnotesize{10} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{22}}\\
\footnotesize{11} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{20}}\\
\footnotesize{12} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{18}}\\
\footnotesize{13} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{16}}\\
\footnotesize{14} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{14}}\\
\footnotesize{15} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{12}}\\

\bottomrule
\end{tabularx}
\caption{Multiple price list of 4-week saving contracts starting at Session 1 (MPL4)}
\label{tab:MPLIV}
\end{table}


\begin{table}[htp]
\begin{tabularx}{\textwidth}{
    c
    @{\hspace{36pt}}
    C{0.1cm} 
  >{\centering\arraybackslash}X 
    C{0.1cm} 
  >{\centering\arraybackslash}X 
    C{0.1cm}
    }
\toprule
 & & \multicolumn{3}{c}{\textbf{Late saving contracts}} & \\
\cline{3-5}
\textbf{Choice} & & \makecell{\small{ Session 2 } \\[-0.2cm] \footnotesize{ (in 4 weeks) }} & & \makecell{\small{ Session 3 } \\[-0.2cm] \footnotesize{ (in 8 weeks) }} & \\
\hline
\footnotesize{1} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{40}}\\
\footnotesize{2} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{35}}\\
\footnotesize{3} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{31}}\\
\footnotesize{4} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{29}}\\
\footnotesize{5} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{27}}\\
\footnotesize{6} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{25}}\\
\footnotesize{7} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{23}}\\
\footnotesize{8} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{21}}\\
\footnotesize{9} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{19}}\\
\footnotesize{10} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{17}}\\
\footnotesize{11} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{15}}\\
\footnotesize{12} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{13}}\\
\footnotesize{13} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{11}}\\
\footnotesize{14} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{9}}\\
\footnotesize{15} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{7}}\\

\bottomrule
\end{tabularx}
\caption{Multiple price list of 4-week saving contracts starting at Session 2 (MPL5)}
\label{tab:MPLV}
\end{table}



\begin{table}[htp]
\begin{tabularx}{\textwidth}{
    c
    @{\hspace{36pt}}
    C{0.1cm} 
  >{\centering\arraybackslash}X 
    C{0.1cm} 
  >{\centering\arraybackslash}X 
    C{0.1cm}
    }
\toprule
 & & \multicolumn{3}{c}{\textbf{Early debt contracts}} & \\
\cline{3-5}
\textbf{Choice} & & \makecell{\small{ Session 1 } \\[-0.2cm] \footnotesize{ (today) }} & & \makecell{\small{ Session 2 } \\[-0.2cm] \footnotesize{ (in 4 weeks) }} & \\
\hline
\footnotesize{1} & & \footnotesize{Receive an amount of \euro{31}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{2} & & \footnotesize{Receive an amount of \euro{27}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{3} & & \footnotesize{Receive an amount of \euro{24}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{4} & & \footnotesize{Receive an amount of \euro{21}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{5} & & \footnotesize{Receive an amount of \euro{19}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{6} & & \footnotesize{Receive an amount of \euro{17}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{7} & & \footnotesize{Receive an amount of \euro{16}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{8} & & \footnotesize{Receive an amount of \euro{15}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{9} & & \footnotesize{Receive an amount of \euro{14}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{10} & & \footnotesize{Receive an amount of \euro{13}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{11} & & \footnotesize{Receive an amount of \euro{11}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{12} & & \footnotesize{Receive an amount of \euro{9}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{13} & & \footnotesize{Receive an amount of \euro{7}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{14} & & \footnotesize{Receive an amount of \euro{5}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{15} & & \footnotesize{Receive an amount of \euro{3}} & & \footnotesize{Pay an amount of  \euro{15}}\\

\bottomrule
\end{tabularx}
\caption{Multiple price list of 4-week debt contracts starting at Session 1 (MPL6)}
\label{tab:MPLVI}
\end{table}


\begin{table}[htp]
\begin{tabularx}{\textwidth}{
    c
    @{\hspace{36pt}}
    C{0.1cm} 
  >{\centering\arraybackslash}X 
    C{0.1cm} 
  >{\centering\arraybackslash}X 
    C{0.1cm}
    }
\toprule
 & & \multicolumn{3}{c}{\textbf{Late debt contracts}} & \\
\cline{3-5}
\textbf{Choice} & & \makecell{\small{ Session 2 } \\[-0.2cm] \footnotesize{ (in 4 weeks) }} & & \makecell{\small{ Session 3 } \\[-0.2cm] \footnotesize{ (in 8 weeks) }} & \\
\hline
\footnotesize{1} & & \footnotesize{Receive an amount of \euro{33}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{2} & & \footnotesize{Receive an amount of \euro{30}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{3} & & \footnotesize{Receive an amount of \euro{27}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{4} & & \footnotesize{Receive an amount of \euro{24}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{5} & & \footnotesize{Receive an amount of \euro{22}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{6} & & \footnotesize{Receive an amount of \euro{20}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{7} & & \footnotesize{Receive an amount of \euro{18}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{8} & & \footnotesize{Receive an amount of \euro{16}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{9} & & \footnotesize{Receive an amount of \euro{15}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{10} & & \footnotesize{Receive an amount of \euro{14}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{11} & & \footnotesize{Receive an amount of \euro{12}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{12} & & \footnotesize{Receive an amount of \euro{10}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{13} & & \footnotesize{Receive an amount of \euro{8}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{14} & & \footnotesize{Receive an amount of \euro{6}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{15} & & \footnotesize{Receive an amount of \euro{3}} & & \footnotesize{Pay an amount of  \euro{15}}\\

\bottomrule
\end{tabularx}
\caption{Multiple price list of 4-week debt contracts starting at Session 2 (MPL7)}
\label{tab:MPLVII}
\end{table}

\begin{comment}
\begin{table}[htp]
\begin{tabularx}{\textwidth}{
    c
    @{\hspace{36pt}}
    C{0.1cm} 
  >{\centering\arraybackslash}X 
    C{0.1cm} 
  >{\centering\arraybackslash}X 
    C{0.1cm}
    }
\toprule
 & & \multicolumn{3}{c}{\textbf{Long saving contracts}} & \\
\cline{3-5}
\textbf{Choice} & & \makecell{\small{ Session 2 } \\[-0.2cm] \footnotesize{ (in 4 weeks) }} & & \makecell{\small{ Session 3 } \\[-0.2cm] \footnotesize{ (in 8 weeks) }} & \\
\hline

\footnotesize{1} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{50}}\\
\footnotesize{2} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{45}}\\
\footnotesize{3} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{40}}\\
\footnotesize{4} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{36}}\\
\footnotesize{5} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{34}}\\
\footnotesize{6} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{32}}\\
\footnotesize{7} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{30}}\\
\footnotesize{8} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{28}}\\
\footnotesize{9} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{26}}\\
\footnotesize{10} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{24}}\\
\footnotesize{11} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{22}}\\
\footnotesize{12} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{20}}\\
\footnotesize{13} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{18}}\\
\footnotesize{14} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{16}}\\
\footnotesize{15} & & \footnotesize{Pay an amount of \euro{15}} & & \footnotesize{Receive an amount of  \euro{14}}\\

\bottomrule
\end{tabularx}
\caption{Multiple price list of 8-week saving contracts from starting at Session 1 (MPL8)}
\label{tab:MPLIIX}
\end{table}





\begin{table}[htp]
\begin{tabularx}{\textwidth}{
    c
    @{\hspace{36pt}}
    C{0.1cm} 
  >{\centering\arraybackslash}X 
    C{0.1cm} 
  >{\centering\arraybackslash}X 
    C{0.1cm}
    }
\toprule
 & & \multicolumn{3}{c}{\textbf{Long debt contracts}} & \\
\cline{3-5}
\textbf{Choice} & & \makecell{\small{ Session 1 } \\[-0.2cm] \footnotesize{ (today) }} & & \makecell{\small{ Session 3 } \\[-0.2cm] \footnotesize{ (in 8 weeks) }} & \\
\hline
\footnotesize{1} & & \footnotesize{Receive an amount of \euro{39}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{2} & & \footnotesize{Receive an amount of \euro{35}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{3} & & \footnotesize{Receive an amount of \euro{31}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{4} & & \footnotesize{Receive an amount of \euro{27}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{5} & & \footnotesize{Receive an amount of \euro{24}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{6} & & \footnotesize{Receive an amount of \euro{21}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{7} & & \footnotesize{Receive an amount of \euro{19}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{8} & & \footnotesize{Receive an amount of \euro{17}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{9} & & \footnotesize{Receive an amount of \euro{16}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{10} & & \footnotesize{Receive an amount of \euro{15}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{11} & & \footnotesize{Receive an amount of \euro{13}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{12} & & \footnotesize{Receive an amount of \euro{11}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{13} & & \footnotesize{Receive an amount of \euro{9}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{14} & & \footnotesize{Receive an amount of \euro{9}} & & \footnotesize{Pay an amount of  \euro{15}}\\
\footnotesize{15} & & \footnotesize{Receive an amount of \euro{7}} & & \footnotesize{Pay an amount of  \euro{15}}\\

\bottomrule
\end{tabularx}
\caption{Multiple price list of 8-week debt contracts starting at Session 1 (MPL9)}
\label{tab:MPLIX}
\end{table}
\end{comment}

==> DSM_(arxiv)/TABLES/tab.survey_module.tex <==
%DEBT AVERSION SURVEY MODULE
\begin{table}[t!]
\caption{Debt Aversion Survey Module \label{table:fullmodule}}
\begin{tabularx}{\textwidth}{
    c 
    L{7cm}
    C{3.5cm}
    >{\centering\arraybackslash}X 
}

\toprule
%\textbf{Pred.} 
& \textbf{Question/Item} 
& \textbf{Response} 
& \textbf{Coeff.} \\
\midrule

\multicolumn{2}{l}{\footnotesize{Please rate the following statement:}}
& 
&\\[+4pt]

\footnotesize{\emph{Q1}}
&\footnotesize{\emph{Debt is an integral part of today's life.}}
& \footnotesize{1:~strongly agree - 6:~strongly disagree}
%\rdelim\}{2.5}{3.5cm}[\makecell{
%\footnotesize{1: strongly agree } \\[-3pt] \footnotesize{6: strongly disagree}}] 
& \footnotesize{$0.0045$} \\[+16pt]

%\footnotesize{\emph{Q2}}
%&\footnotesize{\emph{I feel OK borrowing money for ‘essential’ purchases e.g. cars, appliances, mortgage.}}
%& \footnotesize{1:~very much like me - 6:~not at all like me}
%& \footnotesize{$-0.0049$} \\[+16pt]

\cline{1-2}
\multicolumn{2}{l}{\footnotesize{What do you think, how does the average participant in  }}
&
&\\[-4pt]
\multicolumn{2}{l}{\footnotesize{this survey/experiment rate the following statement: }}
& 
&\\[+4pt]

\footnotesize{\emph{Q2}}
&\footnotesize{\emph{There is no excuse for borrowing money.}}
& \footnotesize{1:~strongly agree - 6:~strongly disagree}
& \footnotesize{$-0.0067$} \\[+16pt]

%\cline{1-2}

%\footnotesize{\emph{Q4}}
%&\footnotesize{\emph{How certain are you about the amount of your overall outstanding debt as of today?}}
%& \footnotesize{1:~very uncertain - 6:~very certain}
%& \footnotesize{$-0.0060$} \\[+16pt]

\cline{1-2}


\footnotesize{\textit{Constant}} 
& 
& 
& \footnotesize{$1.0694$} \\

\bottomrule

%\multicolumn{4}{l}{\scriptsize{Standard errors in parentheses}}\\[-9pt]
%\multicolumn{4}{l}{\scriptsize{$^*p<0.10$; $^{**}p<0.05$; $^{***}p<0.01$}}

\end{tabularx}
\end{table}





\begin{comment}
% Old version containing five items
\toprule
%\textbf{Pred.} 
& \textbf{Question/Item} 
& \textbf{Response} 
& \textbf{Coeff. ($\beta$)} \\
\midrule

\multicolumn{2}{l}{\footnotesize{Please rate the following statements according to your }}
&
&\\[-4pt]
\multicolumn{2}{l}{\footnotesize{own level of agreement: }}
& \rdelim\}{12}{3.5cm}[\makecell{\footnotesize{6-point Likert Scale}\\
\footnotesize{1: strongly agree } \\[-3pt] \footnotesize{6: strongly disagree}}] 
&\\[+4pt]
\cline{1-2}

\footnotesize{\emph{Q1}}
&\footnotesize{\emph{Debt is an integral part of today's life.}}
& 
& \footnotesize{$0.0066$} \\[+4pt]

\footnotesize{\emph{Q2}}
&\footnotesize{\emph{It is okay to accrue debt for living the style you desire.}}
& 
& \footnotesize{$0.0078$} \\[+4pt]

\footnotesize{\emph{Q3}}
&\footnotesize{\emph{I feel OK borrowing money for ‘essential’ purchases e.g. cars, appliances, mortgage.}}
& 
& \footnotesize{$-0.0046$} \\[+16pt]

\multicolumn{2}{l}{\footnotesize{What do you think, how does the average participant }}
&
&\\[-4pt]
\multicolumn{2}{l}{\footnotesize{in this experiment/survey rate the following statement: }}
&
&\\[+4pt]
\cline{1-2}

\footnotesize{\emph{Q4}}
&\footnotesize{\emph{You should always save up first before buying something.}}
& 
& \footnotesize{$-0.0093$} \\[+4pt]

\footnotesize{\emph{Q5}}
&\footnotesize{\emph{You should rather restrict your lifestyle than go into debt.}} 
& 
& \footnotesize{$0.0067$}  \\[+16pt]

\cline{1-2}
\footnotesize{\textit{Constant}} 
& 
& 
& \footnotesize{$1.0080$} \\

\bottomrule
\end{comment}

==> FIGURES/fig.module_selection_slides.tex <==
\begin{figure}[t!]
%\caption{Performance metrics of the candidate survey modules
%\label{fig.performance}}


\begin{subfigure}{1\textwidth}
\begin{minipage}{0.49\textwidth}
\begin{tikzpicture}
\centering
    \hspace{9pt}
	%%%%% ADJUSTED COEFFICIENT OF DETERMINATION
	\begin{axis}[
		width  = 0.95*\textwidth,
		height = 5.5cm,
		ymin=0,
		ymax=0.5,
		axis lines = left,
		ylabel = \footnotesize{adjusted $R^2$},
		ymajorgrids = true,
		xmin = 0,
		xmax = 16,
		tick label style={font=\footnotesize},
		%xlabel= No. of predictors,
		]
        \addplot [red,very thick] table [x="n_tuple", 
                                        y="adj.r.squared.1", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [darkgray] table [x="n_tuple",
                                        y="adj.r.squared.2", 
                                        col sep=comma, 
                               mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray] table [x="n_tuple", 
                                        y="adj.r.squared.3", 
                                        col sep=comma, 
                               mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray, densely dotted] table [x="n_tuple",
                                        y="adj.r.squared.4", 
                                        col sep=comma, 
                               mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [lightgray, dotted] table [x="n_tuple",
                                        y="adj.r.squared.5", 
                                        col sep=comma, 
                               mark=none] {RESULTS/survey_module_selection.csv};
        \addplot[blue, ultra thick, draw opacity=0.1]coordinates{(13,0) (13,0.361038)};
	\end{axis}
\end{tikzpicture}
\end{minipage}
%
\begin{minipage}{0.49\textwidth}
\begin{tikzpicture}
\centering
    \hspace{9pt}
	%%%%% AKAIKE INFORMATION CRITERION
	\begin{axis}[
		width  = 0.95*\textwidth,
		height = 5.5cm,
		ymin=-570,
		ymax=-542,
		axis lines = left,
		ylabel = \footnotesize{AIC},
		ymajorgrids = true,
		xmin = 0,
		xmax = 16,
		tick label style={font=\footnotesize},
		legend entries={\scriptsize{Top1}, \scriptsize{Top2},                                    \scriptsize{Top3},
                        \scriptsize{Top4}, \scriptsize{Top5}},
        legend style={at={(0.975,0.975)}},
		%xlabel= No. of predictors,
		]
        \addplot [red,very thick] table [x="n_tuple",
                                        y="AIC.1", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [darkgray] table [x="n_tuple",
                                        y="AIC.2", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray] table [x="n_tuple",
                                        y="AIC.3", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray, densely dotted] table [x="n_tuple", 
                                        y="AIC.4", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [lightgray, dotted] table [x="n_tuple", 
                                        y="AIC.5", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot[blue, ultra thick, draw opacity=0.1]coordinates{(10,-570) (10,-565.841)};
	\end{axis}
\end{tikzpicture}
\end{minipage}
\end{subfigure}

\vspace{1cm}
\begin{subfigure}{1\textwidth}
\begin{minipage}{0.49\textwidth}
\begin{tikzpicture}
\centering
	%%%%% BAYESIAN INFORMATION CRITERION
	\begin{axis}[
		width  = 0.95*\textwidth,
		height = 5.5cm,
		ymin=-548,
		ymax=-523,
		xlabel= No. of predictors,
		axis lines = left,
		ylabel = \footnotesize{BIC},
		ymajorgrids = true,
		xmin = 0,
		xmax = 16,
		tick label style={font=\footnotesize}
		%xlabel= No. of predictors,
		]
        \addplot [red,very thick] table [x="n_tuple", 
                                        y="BIC.1", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [darkgray] table [x="n_tuple", 
                                        y="BIC.2", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray] table [x="n_tuple", 
                                        y="BIC.3", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray, densely dotted] table [x="n_tuple", 
                                        y="BIC.4", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [lightgray, dotted] table [x="n_tuple", 
                                        y="BIC.5", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot[blue, ultra thick, draw opacity=0.1]coordinates{(1,-548) (1,-544.05)};
	\end{axis}
\end{tikzpicture}
\end{minipage}
%
\begin{minipage}{0.49\textwidth}
\begin{tikzpicture}
\centering
	%%%%% CROSS VALIDATION (k=10)
	\begin{axis}[
		width  = 0.95*\textwidth,
		height = 5.5cm,
		ymin=0.0006,
		ymax=0.00089,
		axis lines = left,
		ylabel = \footnotesize{MSE (CV with k=10)},
		ymajorgrids = true,
		xmin = 0,
		xmax = 16,
		xlabel= No. of predictors,
		scaled ticks=false, 
		tick label style={font=\footnotesize},
		y tick label style={/pgf/number format/.cd,
        fixed,
        fixed zerofill,
        precision=4,
        yticklabels={,,.0007,.0008,},
        /tikz/.cd
        }
		]
        \addplot [red,very thick] table [x="n_tuple", 
                                        y="MSPE_k10_rd100.1", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [darkgray] table [x="n_tuple", 
                                        y="MSPE_k10_rd100.2", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray] table [x="n_tuple", 
                                        y="MSPE_k10_rd100.3", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [gray, densely dotted] table [x="n_tuple", 
                                        y="MSPE_k10_rd100.4", 
                                        col sep=comma,
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot [lightgray, dotted] table [x="n_tuple", 
                                        y="MSPE_k10_rd100.5", 
                                        col sep=comma, 
                                        mark=none] {RESULTS/survey_module_selection.csv};
        \addplot[blue, ultra thick, draw opacity=0.1]coordinates{(8,0.000664) (8,0.0006)};
	\end{axis}
\end{tikzpicture}
\end{minipage}
\end{subfigure}
\vspace{1cm}
\end{figure}
